Integer Forcing: Effective SNR Distribution and Practical Block-Based Schemes

Integer Forcing (IF) is a novel linear receiver architecture, where instead of separating the codewords sent by each transmitter, and decoding them individually, forces integer-valued linear combinations at each receive antenna, and decodes the linear combinations. The original codewords are obtained by inverting the integer-valued matrix. While demonstrating superior performance, IF requires complex optimization in order to find the optimal linear combinations, and demands either using multi-level nested lattice codes, or reducing the rates of all transmitters to equal the weakest one. Finally, the distribution of the resulting effective SNR is hard to evaluate. In this paper, we first give simple upper and lower bounds on the effective SNR of a single linear combination in IF. These expressions allow us to easily bound the distribution of the effective SNR for any given linear combination used. We then suggest two simple block-based IF schemes. These schemes, while sub-optimal, significantly reduce the complexity of the optimization process, and, more importantly, do not require reducing the rates of all transmitters, as decoding is done block-wise. Finally, we bound the distribution of the effective SNR of the decoding schemes, and show via simulations the superiority of block-wise schemes at low SNR.

==> tex_files/0_header_and_titlepage/titlepage.tex <==
\begin{titlepage}
	{\scshape\LARGE 
	\begin{center}
	BEN-GURION UNIVERSITY OF THE NEGEV
	FACULTY OF ENGINEERING SCIENCES
	DEPARTMENT OF COMMUNICATION
SYSTEMS ENGINEERING
\end{center}
 \par}
	\vspace{1cm}
	{\LARGE\bfseries 
	\begin{center}
	Integer-Forcing for Blocks
	\end{center}
	\par}
	\vspace{2cm}
	
	%\begin{center}
	%By: Ron Meiry
	%\end{center}
	%\par
	%\begin{center}
	%Supervised by: Dr. Asaf Cohen and Dr. Omer Gurewitz
%\end{center}
	\vfill
% Bottom of the page
	{\large 
	\begin{center}
	\today
	\end{center}
	\par}
\end{titlepage}


==> tex_files/1_preliminaries/general_background/IF.tex <==

				

\subsection{IF Introduction}\label{sc:IF_intro}

\begin{figure}[htbp]
	\centering
		\includegraphics[width=0.4\textwidth]{dependencies/fig/IF_scheme_sketch/IF_scheme.pdf}
	\caption{IF scheme block diagram} 
	\label{fig:IF_scheme}
\end{figure}

The key idea of the IF \cite{zhan2014integer} linear receiver is to look at linear combinations of codewords (combined-code-words), as a new codeword, and decode it. The coefficients of the combinations are represented as elements of the matrix $\bA$, and are chosen by the receiver, according to the channel state.  The IF receiver requires CSI only at the receiver. In \emph{compute-and-forward} \cite{nazer2011compute}, which is the building block of IF, it is shown how to receive and decode combined-code-words (vectors), instead of the original ones. The codewords are taken from a lattice code book \cite{zamir2014lattice}, and each vector is a codeword by itself, hence, can be decoded (the noise is removed at the decoding process) by its own. After the recovery process, the transmitted vector can be found iff all the vectors together can be inverted. I.e., the vectors construct a full rank matrix $\bA$. The information gathering of the codewords is a digital process which involves finding $\bA^{-1}$ for the recovery. When looking at a vector, the codewords it is built from do not counted as an interference, but as a part of a new codeword (vector) to be decoded. 
Let:  
\begin{align*}
	 \by = \bH\bx + \bz
\end{align*}
Where,  for example: 
\begin{align*}
&\bx = \begin{bmatrix}
  x_1 \\
	x_2
\end{bmatrix}
& 
\bH = 
\begin{bmatrix}
  \bh_1 || \bh_2
\end{bmatrix} = 
\begin{bmatrix}
  2 & 1 \\
	1 & 1
\end{bmatrix} 
& & \bz = 
\begin{bmatrix}
  z_1 \\
	z_2
	\end{bmatrix}.
\end{align*}
$\bx$ are the codewords with a transition power $P$, $\bH$ is the channel matrix, $\bz$ is the noise vector  at the receiver, with variance 1, and $\by$ is the received vector. Then, $\ba$ may be chosen as following:
\begin{align*}
\ba_1 = \begin{bmatrix}2 & 1\end{bmatrix}^T && 
\ba_2 = \begin{bmatrix}1 & 1 \end{bmatrix}^T &&
\bA\in \R^{2 \times 2} = \begin{bmatrix}\ba_1 , \ba_2\end{bmatrix}.
\end{align*}	
 IF may decode:
\begin{align*}
\tilde{\by}_{if} & = \bH\bx + \bz \\
&= \bA\bx +  \underbrace{(\bH-\bA)\bx + \bz}_{\bz_{eff}} 
 =  \bA\bx + \bz_{eff}\\
 &=
 \begin{bmatrix}
  \ba_1^T\bx + z_{eff,1}\\
	\ba_2^T\bx + z_{eff,2}
	\end{bmatrix} =
\begin{bmatrix}
  2 \bx_1 +  \bx_2 + z_1 \\
\bx_1 + \bx_2 +z_2
	\end{bmatrix}.
\end{align*}
Here $\bz_{eff}$,the effective noise vector seen by the decoder, equals $\bz$ because $\bA=\bH$. Since the noise is the same, it's variance remains the same, which is $1$. The ratio between the signal power to the effective noise for both first, and second vectors is:
$\frac{P\cdot 2^2+P \cdot 1^2}{1} = 5P$ for the first. And $\frac{P \cdot 1^2+P\cdot1 ^2}{1}=2P$ for the second. 
When using ZF decoding on the other hand, we get:
\begin{align*}
\begin{bmatrix}
  \tilde{y}_{zf,1} \\
	\tilde{y}_{zf,2} 
	\end{bmatrix} &=
 \tilde{\by}_{zf} = \bH^{-1}\by = \bx + \bH^{-1}\bz\\
& = \bx+\begin{bmatrix}
  1 	& -1 \\
	-1 	& 2
	\end{bmatrix}\bz 
	=\begin{bmatrix}
   x_1\\
	x_2\\
	\end{bmatrix} 
	+
	\begin{bmatrix}
   z_1 - z_2\\
	-z_1+2z_2\\
	\end{bmatrix} 
\end{align*}
The effective SNR for the first vector here  is $\frac{P}{1^2+1^2}=\frac{P}{2}$ while for the second it is $\frac{P}{1^2+2^2}= \frac{P}{5}$. Note the ratio between the best effective SNR for ZF and the worst effective SNR for IF is $2P / \frac{P}{2} = 4$. Hence, for this channel, IF achieves a much better rate compared to ZF, thus, it gives us motivation to use IF. 


\subsection{Architecture Overview}
When using linear receiver such as ZF and MMSE, the output channel ($\by$  for one transmission and $\bY$ for $n$) is inserted to a matrix $\bB$. It's goal is to invert the channel such that each stream can be encoded alone. The other streams are considered as interference. The multiplying of the channel output by $\bB$ amplifies the power for the noise according to the vectors of $\bB$. This amplification might decrease the achievable rate, especially when $\bH$ is an ill-conditioned matrix. Note that ''inverting'' the channel, basically  means to apply linear action such that the channel becomes the identity matrix ($\bI_{M_T}$). The strength of IF is in it's ability to choose any full rank matrix $\bA$ and use $\bB$ to transform the channel into $\bA$. Note that since $\bI$ is a full rank matrix as well, both ZF and MMSE can be achieved by IF. In fact, as explained in \cite{zhan2014integer}, any linear receiver is a special case of IF. 

The intuition for the usage of any full rank $\bA$ and not just $\bI$, comes from the fact that a lattice codebook is used, hence, any linear combination of codewords is a codeword by itself. A lattice codebook is simply a code whose codewords are elements of a lattice \cite{zamir2014lattice}.  The vectors of $\bA$ are the coefficients of this linear combination. After all the linear combination have been decoded, by inverting $\bA$ each codeword can be found. The main trick in IF, is choosing a good $\bA$.

Consider the channel of the $m^{th}$ receive antenna,
\begin{align*}
\by_m^T=\bh_m^T\bX+\bz_m^T.
\end{align*}
and let $\ba_m \in \bA = [a_{m,1},\ldots,a_{m,M_T}]^T$ the desired coefficients vector of the $m^{th}$ antenna. After scaling $\by_m$ by any $\beta_m \in \R$ we have:
\begin{align*}
\tilde{\by}_m = \beta_m \by_m^T= \underbrace{\ba_m^T\bX}_{\text{lattice codeword}} +  \underbrace{(\beta_m\bh_m^T-\ba_m^T)\bX + \beta_m\bz_m^T}_{\text{effective noise}}.
\end{align*}
The variance of the effective noise is:
\begin{align}\label{eq:eff_noise_var}
\sigma_{eff,m}^2 &= \frac{1}{n}\EE[{\normSqr[(\beta_m\bh_m^T-\ba_m^T)\bX + \beta_m\bz_m^T]}] \\
&\stackrel{\eqref{eq:power_constraint_TX}}{=} \underbrace{\beta_m^2}_{\text{amplified noise var.}} + \underbrace{P\normSqr[\beta_m\bh_m-\ba_m]}_{\text{quantization penalty}}.
\end{align}
The $m^{th}$ effective channel output $\tilde{\by}_m$ and it's desired integer coefficient vector $\ba_m$ are fed into a SISO decoder $\mathcal{D}_m : \R^n \times \Z^{M_T} \rightarrow \Z_p^k$. This decoder estimates $\tilde{\bu}_m = \mathcal{D}_m (\tilde{\by}_m, \ba_m)$, for the linear combination defined by $\ba_m$,
\begin{align*}
\bu_m = \left[ \sum_{l=1}^{M_T}a_{m,l}\bw_l  \right] \bmod p.
\end{align*}
Let $\bU = [\bu_1, \ldots, \bu_{M_T}]$, then, if there are no errors, the original codewords $\bW = [\bw_1, , \ldots,  \bw_{M_T}]$ can be found from $\bU$ by:
\begin{align}
\bW = [\bA^{-1}\bU] \bmod p,
\end{align}
where $\bA^{-1}$ is the inverse of $\bA$ over $\Z_p$.
The desired linear combinations can be recovered reliably if the rates do not exceed the rates in the following lemma:
\begin{lemma}[{\cite{nazer2011compute}, Theorem 1}] $\forall \epsilon >0$ and $n,p$ large enough, there exist encoders and decoders, $\mathcal{E}_1,\ldots, \mathcal{E}_{M_T}, \mathcal{D}_1,\ldots, \mathcal{D}_{M_T}$, such that the decoders can recover the linear combination $\bu_m= \left[ \sum_{l} a_{m,l}\bw_l  \right] \bmod p$ from the channel outputs, with total probability of error at most $\epsilon$ for any choice of integer coefficient vectors $\{ \ba_i\}_{i=1}^{M_T} \in \Z^{M_T}$ satisfying
\begin{align*}
 \frac{1}{2}\posLog[\frac{P}{\beta_m^2+P\normSqr[\beta_m\bh_m-\ba_m]}],
\end{align*}
where $\posLog[x] \defined \max\{\Log[x],0\}$.
\end{lemma}
In fact, as can be found in \cite{zhan2014integer}, instead of multiply the $m^{th}$ vector in a scalar $\beta_m$, the entire output can be multiplied in a matrix $\bB = [\bb_1, \ldots, \bb_{M_T}] \in \R^{M_T \times M_R}$ and use the matrix $\bA =  [\ba_1, \ldots, \ba_{M_T}] \in \Z^{M_T \times M_T}$. In that case, the computation rate is a vector and it's  $m^{th}$ element is
\begin{align}\label{eq:computation_rate}
\left[R_{comp}(\bH,\bA,\bB)\right]_m = \frac{1}{2}\posLog[\frac{P}{\normSqr[\bb_m]+P\normSqr[\bH^T\bb_m-\ba_m]}].
\end{align}
Note that the variance of the effective noise, \cref{eq:eff_noise_var}, becomes:
\begin{align}\label{eq:eff_noise_var_after_mult_by_vector}
\sigma_{eff,m}^2 = \bb_m^2 +P\normSqr[\bH^T\bb_m-\ba_m]
\end{align}

\begin{remark}
There is a balance between both terms in \eqref{eq:computation_rate}. For high values of $P$, the quantization penalty becomes very important. Hence, we should allow the noise to be amplified in order to decrease the quantization penalty. However, when $P$ takes very small values, the amplified noise becomes the more significant part, and there is more tolerance for high quantization penalty. This is an optimization problem.\\
\end{remark}

\begin{claim}[\cite{zhan2014integer}. Lemma 3]
For any matrix $\bB$, the architecture above can match the achievable rate of any conventional linear receiver   $R_{linear,m}(\bH,\bB)$ by setting $\bA=\bI$ and by choosing $\tilde{\bB}$ such that $\tilde{\bb_m^T} = \alpha_m\bb_m^T,$ where  
\begin{align*}
\alpha_m = \frac{P\bb_m^T\bh_m}{\normSqr[\bb_m]+P\sum_{i=1}^{M_T}(\bb_m^T\bh_i)^2}.
\end{align*}
Concluding that
\begin{equation*}
R_{linear,m}(\bH,\bB) = \left[R_{comp}(\bH,\bA,\tilde{\bB})\right]_m.
\end{equation*}
\end{claim} 

% 
% \eqref{eq:computation_rate} 


In \cite[Theorem 3]{zhan2014integer}, it is shown that given $\bA$, the optimal $\bB$ and $\bb_m$ are 
\begin{align}
\bB_{opt} 	&= \bA\bH^T\left( \frac{1}{P}\bI +  \bH\bH^T \right)^{-1}\label{eq:B_opt}\\
\bb_{m,opt}^T	&= \ba_m^T\bH^T\left( \frac{1}{P} \bI + \bH\bH^T \right)^{-1}\label{eq:b_opt}
\end{align}
Hence, by setting $\bB$ as in \eqref{eq:B_opt}, the computation rate becomes a function of $\bH,\bA$ and $P$.
The effective SNR's $m^{th}$ element \cite[eq.(10)]{ordentlich2015precoded} becomes
\begin{align}
SNR_{eff,m} \defined SNR_{eff}(\bH,\ba_m) = \frac{1}{\ba_m^T \left(\bI+P\bH^T\bH\right)^{-1}\ba_m}. \label{eq:effective_snr}
\end{align}

When different rates are allowed as happens in CnF, those rates are 
\begin{equation}\label{eq:com_rate_mth_ant}
\left[R_{comp}(\bH,\bA) \right]_m= \frac{1}{2}\log SNR_{eff,m}.
\end{equation}
For IF on the other hand, the same codebook is used by all, thus, all the rates should be equal. The transmission rate becomes 
\begin{align}\label{eq:IF_rate}
 R_{IF}(\bH,\bA) = \min_{m= 1,\ldots,M_T}\left[R_{comp}(\bH,\bA)\right]_m,
\end{align}
hence, the sum rate of IF is 
\begin{equation}
IF_{sum-rate}(\bH,\bA) = M_T \cdot  R_{IF,m}(\bH,\bA).
\label{eq:IF_sum_rate}
\end{equation}


Note that given $\bH$, the rates of both IF and CnF depend \textbf{only} in $\bA$. That means, the 'only' thing  to be done is finding appropriate $\bA$. The problem is, that finding $\bA_{opt}$ for the general case might be difficult. %The search space is exponential in the amount of transmissions and polynomial in the transmission power.
 In order to make the search of $\bA$ more efficient, the following constraint on $\bA$ vectors, \cite[Corollary 2]{zhan2014integer}, can be used:
	\begin{equation}
\label{eq:normConstrintLowP}
		\forall \ba_k\in\bA: \|\ba_k\|<1+\sqrt{P}\cdot\lambda_{max}(\bH),
	\end{equation} 	
	where $\lambda_{max}(\bH)$ is the biggest eigenvalue of $\bH\bH^T$.




==> tex_files/1_preliminaries/general_background/general_background.tex <==
\section{General Background}
In this section, we provide general information and background relevant to the entire work. The \nameref{ssc:MIMO} model is presented. In particular, we discuss the \nameref{ssc:ZF} and The \nameref{ssc:MMSE} linear receivers as conventional receivers for MIMO. We also briefly describe \nameref{sc:lattice_and_nested_lattice} codes. Finally, we examine results on the \nameref{sc:WD} that are useful for performance analysis. 


\input{tex_files/2_preliminaries/general_background/wireless_channels}



==> tex_files/1_preliminaries/general_background/lattice.tex <==
\subsection{Lattice and Nested Lattices}\label{sc:lattice_and_nested_lattice}
\begin{definition}\label{def:lattice_is_close}
[Lattice] An $n$-dimensional lattice $\Lambda$, is a set of points in $\R^{n}$ such that if $\bx\in \Lambda(\bB)$, then $-\bx \in \Lambda$. If also $\bt \in \Lambda$, then $\bx+\bt \in \Lambda$. A lattice can always be written in terms of a lattice generator matrix $\bB \in \bR^{n \times n}$
\begin{align}
\Lambda = \Lambda(\bB) = \{\bx= \bB\bc : \bc\in\Z^n\}.
\end{align}
\end{definition}




\begin{definition}[Quantizer]
A lattice quantizer is a map $Q_\Lambda : \R^n \rightarrow \Lambda$, that sends a point $\bx$ to the nearest lattice point in Euclidean distance
\begin{align}
Q_\Lambda(\bx) = \arg \min \|\bx - \lambda \|.
\end{align}
\end{definition}

\begin{definition}[Voronoi Region]
The fundamental Voronoi region, $\mathcal{V}$, of a lattice, is the set of all points in $\R^n$ that are closest to the zero vector: $\mathcal{V} = \{\bx : Q_\Lambda(\bx) = \textbf{0} \}$. Vol($\mathcal{V}$) denotes the volume of $\mathcal{V}$.
\end{definition}

\begin{definition}[Modulus]
Let $[\bx]\bmod \Lambda$ denote the quantization error of $\bx \in \R^n$ with respect to the lattice $\Lambda$
\begin{align}
[\bx]\bmod \Lambda = \bx - Q_\Lambda(\bx)
\end{align}
\end{definition}
\noindent
$\forall \bx,\bt \in \R^n$ and $\Lambda \subseteq \Lambda_1$, the $\bmod \Lambda$ operation satisfies
\begin{align}
[\bx + \bt] \bmod \Lambda 			&= [[\bx] \bmod \Lambda + \bt] \bmod \Lambda\\
[Q_\Lambda(\bx)] \bmod \Lambda  &= [Q_{\Lambda_1} ([\bx] \bmod \Lambda)] \bmod \Lambda\\
\forall a\in\Z: [a\bx] \bmod \Lambda 						&= [a[\bx] \bmod \Lambda] \bmod \Lambda \\
\forall \beta \in\R: \beta[\bx] \bmod \Lambda 	&= [\beta\bx] \bmod \beta\Lambda \label{eq:lattice_scaling}
\end{align}
Consider a codebook were the codewords are all the points of a lattice $\Lambda$. Since any linear combination of codewords is a codeword as well, a lattice codebook is basically a linear codebook. This attribute is important, since the linear codebook property is used to decode linear combinations of codewords, instead of  just the original transmitted codewords.


\begin{definition}[Nested Lattice]\label{def:nested_lattice}
A lattice $\Lambda$ is said to be nested in a lattice $\Lambda_1$ if $\Lambda \subseteq \Lambda_1$. A sequence of lattices $\Lambda,\Lambda_1,\ldots,\Lambda_L$ is nested if $\Lambda \subseteq \Lambda_1 \subseteq\ldots \subseteq \Lambda_L$.
\end{definition}

\begin{definition}[Nested Lattice Codes]
A nested lattice code $\mathcal{L}$ is the set of all points of a fine lattice $\Lambda_1$ that are within the fundamental Voronoi region $\mathcal{V}$ of a coarse lattice $\Lambda$;
\begin{align*}
\mathcal{L} = \Lambda_1 \cap \mathcal{V} = \{ \bt : \bt = \lambda \bmod \Lambda, \lambda \in \Lambda_1 \}.
\end{align*}
The rate of a nested lattice code is
\begin{align*}
r = \frac{1}{n}\log|\mathcal{L}| = \frac{1}{n}\log\frac{Vol(\mathcal{V})}{Vol(\mathcal{V}_1)}.
\end{align*}
\end{definition}
Nested lattice codes become useful when different streams transmit at different rates. The more dense a lattice is, the smaller it's  Voronoi Region.

For some intuition about the decoding process of nested lattices, let us assume that two codewords $c_1\in \Lambda_1$  and $c_2\in \Lambda_2$ such that $\Lambda_1 \subseteq \Lambda_2$ are transmitted over a noiseless channel with integer gains and two receiving antennas $y_1,y_2$.  Let
\begin{align*}
&\bx = [c_1,c_2]^T \in \Lambda_1 \times \Lambda_2\\
&\by = [y_1,y_2]^T\\
&\bH = \begin{bmatrix}
  h_{11} 	& h_{12} \\
	h_{21} 	& h_{22} 
	\end{bmatrix}\in \Z^{2\times 2}\\
&\det(\bH) =d
\end{align*}
where $d \neq 0$. Without loss of generality, we assume that 
\begin{equation}
d>0 \Longrightarrow d \in \N \Longrightarrow h_{11}h_{22}-h_{12}h_{21} \in \N.
\end{equation} 
 The channel above is given by 
\begin{align*}
\begin{bmatrix}
  y_{1}\\
	y_{2}
	\end{bmatrix}=\by = \bH\bx =
	\begin{bmatrix}
  h_{11}c_1+ h_{12}c_2\\
	h_{21}c_1+ h_{22}c_2
	\end{bmatrix}.
\end{align*}
How can we find $\bx$?
First we notice that
\begin{align*}
y_1 &= \underbrace{c_1+\ldots+ c_1}_{h_{11}\text{ times}} + \underbrace{c_2+\ldots+ c_2}_{h_{12}\text{ times}} = \tilde{c_{11}} + \tilde{c_{12}},\\
y_2 &= \underbrace{c_1+\ldots+ c_1}_{h_{21}\text{ times}} + \underbrace{c_2+\ldots+ c_2}_{h_{22}\text{ times}} = \tilde{c_{21}} + \tilde{c_{22}}.
\end{align*}
Let $i \in \{1,2\}$, then, by \Cref{def:lattice_is_close}: $\tilde{c_{i1}}\in \Lambda_1$ and $\tilde{c_{i2}} \in \Lambda_2$. Moreover, since $\Lambda_1 \subseteq \Lambda_2$, we can say that $\tilde{c_{21}},\tilde{c_{22}},\tilde{c_{11}},\tilde{c_{12}} \in \Lambda_2$. According to \Cref{def:lattice_is_close,def:nested_lattice}, both $d \cdot c_1$ and $-d \cdot c_2$ $\in \Lambda_2$. Therefore,
\begin{align}
d\cdot c_1 &= \det(\bH) \cdot c_1   = c_1 \left(h_{11}h_{22} - h_{21}h_{12}\right) = y_1 h_{22}-y_2 h_{12}\label{eq:pre_find_codewords_from_nested_lattice1}\\
 -d\cdot c_2 &=  -\det(\bH) \cdot c_2 =  c_2 \left(h_{21}h_{12}-h_{11}h_{22}\right) =y_1 h_{21} -y_2h_{11}\label{eq:pre_find_codewords_from_nested_lattice2}  
\end{align}
and by \cref{eq:lattice_scaling}, 
\begin{align}\label{find_codewords_from_nested_lattice}
\bx &=\begin{bmatrix}
  c_{1}\\
	c_{2}
	\end{bmatrix} = 
d^{-1}\cdot \begin{bmatrix}
   y_1 h_{22}-y_2 h_{12}\\
	y_2h_{11} - y_1 h_{21} 
	\end{bmatrix}.
\end{align}
Recalling that both $\bH$ and $\by$ are known, we conclude that $\bx$ can be found by \cref{eq:pre_find_codewords_from_nested_lattice1,eq:pre_find_codewords_from_nested_lattice2,find_codewords_from_nested_lattice}. For more information about the decoding process and how it is done in a noisy channel, together with the conditions for a successful decoding and when $[\bH]_{ij} \in \C$, please see \cite{nazer2011compute}.
 



==> tex_files/1_preliminaries/general_background/lattice_total.tex <==
\subsection{Lattice and Nested Lattice}
\subsubsection{Definitions}
\begin{definition}[Lattice] An $n$-dimensional lattice $\Lambda$, is a set of points in $\R^{n}$ such that if $\bs\in \Lambda$, then $-\bs \in \Lambda$. If also $\bt \in \Lambda$, then $\bs+\bt \in \Lambda$. A lattice can always be written in terms of a lattice generator matrix $\bB \in \bR^{n \times n}$
\begin{align*}
\Lambda = \{\bs= \bB\bc : \bc\in\Z^n\}
\end{align*}
\end{definition}

\begin{definition}[Nested Lattice]
A lattice $\Lambda$ is said to be nested in a lattice $\Lambda_1$ if $\Lambda \subseteq \Lambda_1$. We will sometimes refer to $\Lambda$ as the coarse lattice and $\Lambda_1$ as the fine lattice. More generally, a sequence of lattices $\Lambda,\Lambda_1,\ldots,\Lambda_L$ is nested if $\Lambda \subseteq \Lambda_1 \subseteq\ldots \subseteq \Lambda_L$.
\end{definition}


\begin{definition}[Quantizer]
A lattice quantizer is a map $Q_\Lambda : \R^n \rightarrow \Lambda$, that sends a point $\bs$ to the nearest lattice point in Euclidean distance
\begin{align*}
Q_\Lambda(\bs) = \arg \min \|\bs - \lambda \|
\end{align*}
\end{definition}

\begin{definition}[Voronoi Region]
The fundamental Voronoi region, $\mathcal{V}$, of a lattice, is the set of all points in $\R^n$ that are closest to the zero vector: $\mathcal{V} = \{\bs : Q_\Lambda(\bs) = \textbf{0} \}$. Vol($\mathcal{V}$) denotes the volume of $\mathcal{V}$.
\end{definition}

\begin{definition}[Modulus]
Let $[\bs]\bmod \Lambda$ denote the quantization error of $\bs \in \R^n$ with respect to the lattice $\Lambda$
\begin{align*}
[\bs]\bmod \Lambda = \bs - Q_\Lambda(\bs)
\end{align*}
\end{definition}
$\forall \bs,\bt \in \R^n$ and $\Lambda \subseteq \Lambda_1$, the $\bmod \Lambda$ operation satisfies
\begin{align*}
[\bs + \bt] \bmod \Lambda 			&= [[\bs] \bmod \Lambda + \bt] \bmod \Lambda\\
[Q_\Lambda(\bs)] \bmod \Lambda  &= [Q_{\Lambda_1} ([\bs] \bmod \Lambda)] \bmod \Lambda\\
\forall a\in\Z: [a\bs] \bmod \Lambda 						&= [a[\bs] \bmod \Lambda] \bmod \Lambda \\
\forall \beta \in\R: \beta[\bs] \bmod \Lambda 	&= [\beta\bs] \bmod \beta\Lambda \\
\end{align*}

\begin{definition}[Nested Lattice Codes]
A nested lattice code $\mathcal{L}$ is the set of all points of a fine lattice $\Lambda_1$ is the set of all points of a fine lattice that are within the fundamental Voronoi region $\mathcal{V}$ of a coarse lattice $\Lambda$
\begin{align*}
\mathcal{L} = \Lambda_1 \cap \mathcal{V} = \{ \bt : \bt = \lambda \bmod \Lambda, \lambda \in \Lambda_1 \}
\end{align*}
The rate of a nested lattice code is
\begin{align*}
r = \frac{1}{n}\log|\mathcal{L}| = \frac{1}{n}\log\frac{Vol(\mathcal{V})}{Vol(\mathcal{V}_1)}
\end{align*}
Let $\mathcal{B}(r)$ denote an $n$-dimensional ball of radius $r$,
\begin{align*}
\mathcal{B}(r) \defined \{\bs = \|\bs\| \leq r, \bs \in \R^n\}
\end{align*}
and let $\mathcal{B}(r)$ denote its volume.
\end{definition}

\begin{definition}[Covering Radius]
The covering radius of a lattice $\Lambda$ is the smallest real number $r_{COV}$ such that $\R^n \subseteq \Lambda + \mathcal{B}(r_{COV})$.
\end{definition}

\begin{definition}[Effective Radius]
The effective radius of a lattice with Voronoi region $\mathcal{V}$ is the real number $R_{EFFEC}$ that
satisfies $Vol(\mathcal{B}(r_{EFFEC})) = Vol(\mathcal{V})$
\end{definition}

\begin{definition}[Moments]
The second moment of a lattice
is defined as the second moment per dimension of a uniform
distribution over the fundamental Voronoi region $\mathcal{V}$
\begin{align*}
\sigma_\Lambda^2 = \frac{1}{n Vol(\mathcal{V})}\int_{\mathcal{V}}{\normSqr[\bx]d\bx}
\end{align*}
\end{definition}
The normalized second moment of a lattice is given by
\begin{align*}
G(\Lambda) = \frac{\sigma_\Lambda^2}{\left(Vol(\mathcal{V})\right)^{2/n}}
\end{align*}
The following three definitions are the basis for proving
AWGN channel coding theorems using nested lattice codes.
Let $\Lambda^{(n)}$ denote a sequence of lattices indexed by their dimension.

\begin{definition}[Covering Goodness]
A sequence of lattices $\Lambda^{(n)} \subset \R^n$ is good for covering if
\begin{align*}
\lim_{n \rightarrow \infty}\frac{r_{COV}^{(n)}}{r_{EFFEC}^{(n)}}=1
\end{align*}
\end{definition}

\begin{definition}[Quantization Goodness]
A sequence of lattices $\Lambda^{(n)}\subset \R^n$ is good for mean-squared error (MSE) quantization
if
\begin{align*}
\lim_{n \rightarrow \infty}\ G \left( \Lambda^{(n)} \right) = \frac{1}{2\pi e}
\end{align*}
\end{definition}

\begin{definition}[AWGN Goodness] 
Let $\bz$ be a length-$n$ i.i.d Gaussian vector, $\bz \sim \mathcal{N}(0,\sigma_Z^2 \bI_{n \times n})$. The volume-to-noise ratio of a lattice is given by
\begin{align*}
\mu(\Lambda,\epsilon) = \frac{\left( Vol(\mathcal{V}) \right)^{2/n}}{\sigma_Z^2}
\end{align*}
\end{definition}
where $\sigma_Z^2$ is chosen such that $\Pr\{\bz \neq \mathcal{V}\}=\epsilon$. A sequence of lattices $\Lambda^{(n)}$ is good for AWGN if
\begin{align*}
\forall \epsilon 
\in (0,1): \lim_{n\rightarrow \infty} \mu\left( \Lambda^{(n)},\epsilon \right) = 2\pi e
\end{align*}
and, for fixed volume-to-noise ratio greater than $2 \pi e, \Pr\{\bz \neq \mathcal{V}^{(n)} \}$ decays exponentially in $n$

\paragraph{Lattice Constructions}
\begin{lemma}[Erez-Litsyn-Zamir]
There exists a sequence of lattices $\Lambda^{(n)}$ that is simultaneously good for covering, quantization,
and AWGN.
\end{lemma}
The lemma is used to build a lattice code book. The lattice from the lemma scaled such that its second moment is equal to $P$. Let $\bB\in \R^{n \times n}$ denote the generator matrix of this lattice. Our fine lattices are
defined using the following procedure, which is often referred to as Construction A.
\begin{enumerate}
	\item Draw a matrix $\bG_L \in \F_p^{n \times k_L}$ with every element chosen i.i.d. according to the uniform distribution over $\{ 0,1,\ldots, p-1\}$. Recall that $p$ is prime.
	\item Define the codebook $\mathcal{C}_L$ as follows:
	\begin{equation*}
	\mathcal{C}_L = \{\bc = \bG_L\bw : \bw \in \F_p^{k_L}   \}
	\end{equation*}
	All operations in this step are over $\F_p$  
	\item Form the lattice $\tilde{\Lambda}_L$ by projecting the codebook into the reals by $g(\cdot)$, scaling down by a factor of $p$ and placing a copy at every integer vector. This tiles the codebook over $\R^n$
\begin{equation*}
\tilde{\Lambda}_L = p^{-1}g(\mathcal{C}_L)+\Z^n
\end{equation*}
\item  $\tilde{\Lambda}_L$ by the generator matrix of the coarse nested lattice to get the fine lattice for transmitter
\begin{equation*}
\Lambda_L = \bB\tilde{\Lambda}_L
\end{equation*}
\item Repeat steps (1-4) for each transmitter $l = 1,\ldots, L-1$ by replacing $\bG_L$ with $\bG_l$ which is defined to be the first $k_l$ columns of of $\bG_l$
\end{enumerate}
Since $k_1\leq \cdots \leq k_L$,  Any pair of fine lattices $\Lambda_a,\Lambda_b$ when $1 \leq a < b <L$ are nested since all elements of $\mathcal{C}_a$ can be found from $\bG_b$ multiplying by all $\bw \in \F^{n \times k_b}$ with zeros in the last $b-a$ elements. Also observe that $\Lambda = \bB\Z^n$ is nested within each fine lattice by construction. Therefore, the lattices are nested in the desired order, $\Lambda \subseteq \Lambda_1 \subseteq \cdots \subseteq \Lambda_L $.
By choosing $p$ and $k_1,\ldots,k_L$ to grow appropriately with $n$, all the matrices $\bG_1,\ldots,\bG_l$ are full rank with probability that goes to 1 with $n$. Note that if $\bG_l$ has full rank, then the number of fine lattice points in the fundamental Voronoi region $\mathcal{V}$ of the coarse lattice is given by $|\Lambda_l \cap \mathcal{V}|= p^{k_l}$. Hence, the rate of the $l$th nested lattice code $\mathcal{L}_l = \Lambda_l \cap \mathcal{V}$ is 
\begin{equation}
r_l = \frac{1}{n}\log|\Lambda_l \cap \mathcal{V}| = \frac{k_l}{n}\log p = R_l
\end{equation}

\begin{remark}
We require that the fine lattices are generated from full-rank submatrices of the same finite field codebook so that it is possible to compute linear equations over messages with different rates. The full rank condition on the coarse lattice allows us to move between lattice equations and equations of finite field messages.
\end{remark}

	\begin{lemma}[\cite{nazer2011compute}, Lemma 3]
	Let $\Lambda_l(i)$ denote the $i$th point in the $l$th nested lattice code $\mathcal{L}_l = \Lambda_L \cap \mathcal{V}$ for $i = 0,1,\ldots,p^{k_l}-1$ from the
random lattice construction above. We have that:
	\end{lemma}
	\begin{itemize}
		\item $\Lambda_l(i)$ is uniformly distributed over $p^{-1} \Lambda \cap \mathcal{V}$
		\item $\forall i_1 \neq i_2, [\Lambda_l(i_1)-\Lambda_l(i_2)] \bmod \Lambda$ is uniformly distributed over $\{p^{-1}\Lambda\} \cap \mathcal{V}$.
	\end{itemize}
	Thus, each fine lattice can be interpreted as a diluted version of a scaled down coarse lattice $p^{-1}\Lambda$
	
	\paragraph{Integer Combinations of Lattice Points}
	The CnF scheme relies on mapping messages from a finite field to codewords from a nested lattice code. The relay will first decode an integer combination of lattice codewords and then convert this into an equation of the messages. 
	
	\begin{definition}[Lattice Equation]
	A lattice equation $\bv$ is an integer combination of lattice codewords $\bt_l \in \mathcal{L}_l$	modulo the coarse lattice,
\begin{equation*}
\bv = \left[    \sum_{l=1}^L a_l\bt_l\right] \bmod \Lambda
\end{equation*}
for some coefficients $a_l \in \Z$. Note that the lattice equation takes values on the finest lattice
in the summation. That is, if $\forall l: a_l=0$ then the lattice equation $\bv$ only takes values on $\mathcal{L}_L = \Lambda_l \cap \mathcal{V}$.
	\end{definition}
	
	\begin{lemma}[\cite{nazer2011compute}, Lemma 4]
	Any lattice $\Lambda$ that results from Construction A has a full-rank generator matrix $\bB$.
	\end{lemma}

	Since our nested lattice codes are built using nested finite field codes, it is possible to map messages to lattice points and back while preserving linearity. The next two lemmas make this notion precise.
	
	
	\begin{lemma}[\cite{nazer2011compute}, Lemma 5]
	Let $\bW_l$ be a message in $\F_p^{k_l}$ that is zero-padded to length $k$. The function
	\begin{equation*}
\phi(\bw_l) = \left[ \bB p^{-1}g\left(\bG\bw_l\right)   \right] \bmod \Lambda
\end{equation*}
is a one-to-one map between the set of such messages and the elements of the nested lattice code $\mathcal{L}_l = \Lambda_l \cap \mathcal{V}$.
	\end{lemma}
	
\begin{lemma}[\cite{nazer2011compute}, Lemma 6]
Let $\bu =\bigoplus_l q_l\bw_l$ be the desired equation for some coefficients $q_l \in \F_p$ and messages $\bw_l \in \F_p^{k_l}$ zero-padded to length $k$. Assume the messages are mapped to nested lattice codewords, $\bt_l=\phi(\bw_l)$, and let $\bv = \left[ \sum a_l\bt_l  \right] \bmod \Lambda$ denote the lattice equation for some $a_l \in \Z$ such that $q_l = g^{-1}\left([a_l] \bmod p  \right)$.  Then the desired equation can be  obtained using $\bu = \phi^{-1}(\bv)$ where
	\begin{equation*}
\phi^{-1}(\bv) = (\bG^T\bG)^{-1}\bG^T g^{-1}\left(p [\bB^{-1}\bv] \bmod \Z^n\right)
\end{equation*}
	\end{lemma}



==> tex_files/1_preliminaries/general_background/wireless_channels.tex <==

\subsection{Linear Receivers}
%The problem with capacity is it complexity; it can be hard and even impossible to achieve the capacity since an ML receiver is needed. In order to avoid the exponential complexity of ML receiver, it is very common to use linear receivers instead. Such receiver has much better, i.e. polynomial, complexity  in exchange for performance, i.e., achievable rate.
The complexity of Maximum Likelihood decoding on the entire sequence is too high, and prevents the use of simple codes for the SISO channel. To avoid the complexity, linear receivers can be used. A linear receiver decouples the MIMO channels before decoding. Given a channel output $\by$, the receiver may apply an equalization matrix $\bB \in \R^{n_t \times n_r}$ to obtain
\begin{align}\label{eq:linear_receiver_vector}
\tilde{\by} = \bB \by = \bB\bH\bx + \bB\bz.
\end{align}
\Cref{fig:linear_receiver_block_diagram} presents a block diagram of a linear receiver.
\begin{figure}[ht]
	\centering
		\includegraphics[width=0.4\textwidth]{dependencies/fig/linear_receiver_scheme/linear_receiver.pdf}
	\caption{Linear receiver block diagram}
	\label{fig:linear_receiver_block_diagram}
\end{figure}

In order to apply a linear receiver, CSI is needed.
The $k^{th}$ element of $\tilde{\by}$ can be expressed as:
\begin{align}\label{eq:linear_receiver_scalar}
\tilde{y}_k = \bb_k^T \bh_k x_k + \sum_{i \neq k} \bb_k^T \bh_i x_i + \bb_k^T\bz ,
\end{align}
where $\bb_k^T$ is the $k^{th}$  row of $\bB$, $\bh_k$ is the $k^{th}$ column of $\bH$ and $x_k$ is a symbol of the  $k^{th}$ stream. The second and third summands can be viewed as effective noise.
The effective SNR is the ratio between the signal power to the variance of the effective noise at the receiver. The effective SNR of the $k^{th}$ vector is denoted by $SNR_{eff,k}$:
\begin{align}\label{eq:snr_linear_eff_k_No}
 SNR_{linear-eff,k}=\frac{P_k (\bb_k^T\bh_k)^2}{N_o \cdot \normSqr[\bb_k]+\sum_{i\neq k}P_i( \bb_k^T\bh_i)^2}.
\end{align}
In our model, we assume that all the data steams use the same transmission power $P$, and the variance of the noise equals one. By setting $N_0=1$ in \cref{eq:snr_linear_eff_k_No}, the effective SNR becomes:
\begin{align}\label{eq:SNR_eff_linear_receiver_k}
SNR_{linear-eff,k} = \frac{P (\bb_k^T\bh_k)^2}{ \normSqr[\bb_k]+P\sum_{i\neq k}( \bb_k^T\bh_i)^2}
\end{align}
 The rate achieved by the linear receiver for the $k^{th}$ vector is:
\begin{align}\label{eq:linear_receiver_rate}
R_{linear,k}(\bH,\bB) = \Log[1+SNR_{linear-eff,k}].
\end{align}
As we can see, the key idea behind linear receivers is choosing an appropriate $\bB$. The Zero Forcing and the MMSE are two methods to do so.
	\subsubsection{Zero Forcing (ZF)}\label{ssc:ZF}
ZF is a linear receiver, whose goal is to invert the linear combinations forced on the receivers by the channel. When doing so, the original transmitted vector is received, in addition to a noise that is amplified by the inverse operation. Thus, ZF is a linear receiver that uses $\bB=\bH^{\dagger}$, where $\bH^{\dagger} = \left(\bH^*\bH\right)^{-1}\bH^*$ is the pseudoinverse matrix of $\bH$. In that case, the output vector of ZF is:
\begin{equation}
\by_{ZF} = \bH^{\dagger}\by = \bx+\bH^\dagger\bz.
\end{equation}
For more information see \cite[8.3.1]{tse2005fundamentals}. The effective SNR for the $k^{th}$ stream is that case is 
\begin{equation}
SNR_{ZF,k} = \frac{P_k}{N_0\normSqr[\bh^{\dagger}_k]}. 
\end{equation}

As can be found in \cite[(14)-(15)]{jiang2011performance}, the capacity under ZF is:
\begin{equation}
C_{ZF}= \sum_{k=1}^{n_t} \log(1+SNR_{ZF,k}),
\end{equation}
which is basically the sum of the rates for each stream. This is, since after the channel inversion, the streams are orthogonal, hence, do not interfere with each other. When $\frac{P_K}{N_0} \gg 1$, using Taylor series, we have:
\begin{align*}
& \Log[1+\frac{P_k\normSqr[\bh^\dagger_k]}{N_0}] = \Log[\frac{P_k\normSqr[\bh^\dagger_k]}{N_0}] + O\left(\frac{N_0}{P_k\normSqr[\bh^\dagger_k]}\right).
\end{align*} 
%Therefore, we can say that:
%\begin{align*}
%\overline{C}_{ZF,k}
%&\approx \EE[{\Log[\frac{P_k\normSqr[\bh^\dagger_k]}{N_0}]}] = \Log[\frac{P_k}{N_0}]+ \EE[{\Log[{\normSqr[\bh^\dagger_k]}]}]
%\end{align*}  
%For equal power allocation, i.e., $P_k = \frac{P}{n_t} \Longrightarrow \frac{P}{N_0} = P=SNR$ we have:
%\begin{align*}
%\overline{C}_k 
%&\approx \log P + \EE[{\Log[{\normSqr[\bh^\dagger_k]}]}] \\
%&=\log P + \EE[{\Log[{\chi_{2(n_r-n_t+1)}^2}]}] \\
%\end{align*} 
%Where $\EE[{\Log[{\chi_{2(n_r-n_t+1)}^2}]}]$ is the expected value of the log function over a RV with $\chi^2$ distribution. We Conclude that:
%\begin{align*}
 %C_{ZF}
%&\approx \sum_{k} \left(\log P  + \EE[{\Log[{\chi_{2(n_r-n_t+1)}^2}]}] \right)\\
%&= n_t \cdot\left( \log P   +  \EE[{\Log[{\chi_{2(n_r-n_t+1)}^2}]}]\right)\\
%&= n_t \log P  + n_t \EE[{\Log[{\chi_{2(n_r-n_t+1)}^2}]}]
%\end{align*} 
%The first term shows that the ZF achieves the same asymptomatic behavior as the capacity \cite[(8.20)]{tse2005fundamentals}.
%














%The $k^{th}$ data stream can be represented as:
%\begin{align*}
%\by = \sum_{i=1}^{n_t} \bh_i x_i + \bw  = \bh_k x_k  + \sum_{i\neq k} \bh_i x_i + \bw  
%\end{align*}
%In order to remove the inter-stream interference, $\by$ can be projected on an orthonormal subspace, which is orthogonal to the one spanned by $\{\bh_i\}_{i\neq k}$.  This subspace is denoted by $\bV_k$. Since the projection is linear, it can be represented by the matrix $\bQ_k$. Now, each stream can be projected and the inter-stream interference is no longer exists. If $P_k$ is the the power allocated to stream $k$ and $N_0$ is the noise variance then the SNR of the output of this filter is:
%\begin{align*}
%\frac{P_k\normSqr[\bQ_k\bh_k]}{N_0}
%\end{align*} 
%The the $k^{th}$ filter, $c_k$, is given by:
%\begin{align*}
%& \bc_k^* = (\bQ_k\bh_k)^*\bQ_k &\text{or} &
%& \bc_k = (\bQ_k^*\bQ_k)\bh_k
%\end{align*} 
%This is decorrelation of $\bh_k$ over $\bV_k$ expressed in terms of the original coordinates. In fact, applying the decoration filter over all the streams together, can be done by decorrelate the $k^{th}$ stream using the $k^{th}$ column of the $\bH^{\dagger}$, the pseudo-inverse of $\bH$ which is:
%\begin{align*} 
%\bH^{\dagger} \defined \left( \bH^{*}\bH \right)^{-1}\bH^*
%\end{align*} 
%
%
%
%Let $C_k$ be the capacity of the $k^{th}$ stream for a constant channel, which is achieved by a complex Gaussian code book. Then, $C_k = \Log[1+ \frac{P_k\normSqr[\bQ_k\bh_k]}{N_0}]$. 
%As a result, the sum rate achieved by all streams together  is:
%\begin{align*}
%\sum_{k=1}^{n_t}C_k
%\end{align*} 
%For fading channels, the sum rate can be found by averaging over the stationary distribution of the channel.  
%\begin{align*}
%&\overline{C}_k= \EE[{\Log[1+\frac{P_k\normSqr[\bQ_k\bh_k]}{N_0}]}]\\
%& R_{decorr} = \sum_{k} \overline{C}_k
%\end{align*} 
%$\bh_k \sim \mathcal{CN}(0,\bI_{n_r}) \Longrightarrow \normSqr[\bh_k] \sim \chi_{2n_r}^2$. Because $\bQ_k\bQ_k^* = \bI_{dim(\bV_k)}$, we can see why $\normSqr[\bQ_k\bh_k] \sim \chi_{2n_r}^2$ as well. It can be shown that $dim(\bV_k) = n_t -n_r +1$ and when $n_t\geq n_r$, the channel $\bH$ is full rank with probability 1.

%For When $\frac{P_K}{N_0} \gg 1$,by using Taylor series, we have:
%\begin{align*}
%& \Log[1+\frac{P_k\normSqr[\bQ_k\bh_k]}{N_0}] = \Log[\frac{P_k\normSqr[\bQ_k\bh_k]}{N_0}] + O\left(\frac{N_0}{P_k\normSqr[\bQ_k\bh_k]}\right)
%\end{align*} 
%Therefore, we can say that:
%\begin{align*}
%\overline{C}_k 
%&\approx \EE[{\Log[\frac{P_k\normSqr[\bQ_k\bh_k]}{N_0}]}] = \Log[\frac{P_k}{N_0}]+ \EE[{\Log[{\normSqr[\bQ_k\bh_k]}]}]
%\end{align*}  
%For equal power allocation, i.e., $P_k = \frac{P}{n_t} \Longrightarrow \frac{P}{N_0} = P=SNR$ we have:
%\begin{align*}
%\overline{C}_k 
%&\approx \log P + \EE[{\Log[{\normSqr[\bQ_k\bh_k]}]}] \\
%&=\log P + \EE[{\Log[{\chi_{2(n_r-n_t+1)}^2}]}] \\
%\end{align*} 
%Concluding that:
%\begin{align*}
 %R_{decorr} 
%&\approx \sum_{k} \left(\log P  + \EE[{\Log[{\chi_{2(n_r-n_t+1)}^2}]}] \right)\\
%&= n_t \cdot\left( \log P   +  \EE[{\Log[{\chi_{2(n_r-n_t+1)}^2}]}]\right)\\
%&= n_t \log P  + n_t \EE[{\Log[{\chi_{2(n_r-n_t+1)}^2}]}]
%\end{align*} 
%in high SNR, the decorrelator achieves the same amount of DoF as the capacity.








	\subsubsection{Minimum Mean Square Error (MMSE)}\label{ssc:MMSE}
ZF preforms well at high SNR. When the SNR is high, inter-stream interference is much more influential than the noise. In that case, ignoring the noise and using decorrelator to detect the signal is effective. This is the reason the ZF receiver has good performance for high SNR.  On the other hand, the lower the SNR is, the worse the performance of ZF. For the low SNR case, using a matched filter (ignoring the inter-stream interference) achieves much better results, as can be seen in \cite[Figure 8.13]{tse2005fundamentals}. The optimum is a linear receiver that trades off fighting inter-stream interference and the background Gaussian noise. This receiver should maximize the SINR. Thus, this receiver should look like ZF for high SNR, and like matched filter for low. Indeed, the MMSE receiver is given by \cite[(11),(13)]{jiang2011performance}:
\begin{equation}
\bB_{MMSE} = \left(\bH^*\bH + \frac{N_0}{P}\right)^{-1}\bH^*.
\end{equation}
When the ratio between $P$ and $N_0$ is extremely high, $\bB_{MMSE}$ is reduced to $\bB_{ZF} = \bH^\dagger =\left(\bH^*\bH\right)^{-1}\bH^*$. Meaning,  minimizing the \emph{Inter Symbol Interference} (ISI) and ignoring the noise. However, when the ratio between $P$ and $N_0$ becomes extremely small, the ISI becomes negligible compared to the noise, hence, can be ignored. The filtering matrix $\bB_{MMSE}$ behaves as the matrix $\frac{P}{N_0}\bH^*$. Basically,  we can say that by applying $\bB_{MMSE}$, the matched filter is applied on the channel in that case. For farther explanations please see \cite[8.4.3]{biglieri2016academic}. 



\subsubsection{Better Performance Using Successive Interference Cancellation }
One way to achieve better performance of linear receivers is by applying \emph{Successive Interference Cancellation} (SIC).  Let us assume that the recovering process is done by a set of linear decoders, each one is used for the recovery of a single steam. After the first data steam was recovered, in order to recover the second, SIC proceeds as follows: Since the first stream  has already been recovered, it can be subtracted from the channel's output. Now, we have a channel output which is equivalent to the same channel, but with one less transmitter. The action can be applied for the third stream as well, so on. For example, when using the MMSE-SIC, the capacity of the MIMO channel  is achieved, as can be found in \cite[(8.71)]{tse2005fundamentals}. More explanations can be found in \cite[8.3.2]{tse2005fundamentals}.


	\subsubsection{Summary}
Any linear receiver may take the output vector $\by$ and multiply it by a matrix $\bB$. The ZF receiver is a very intuitive linear receiver since it inverts the channel, leaving the receiver with the original signal and amplified noise. \reminder{The ZF maximizes the SNR at the receiver (why it is not true?)} The MMSE, on the other hand, maximizes the SINR and preforms at least as good as the ZF for any channel. When the transmission power is relatively high, for example when  $P \rightarrow \infty$, the  ZF and the MMSE performances are almost the same. However, when the transmission power is relatively small, the performance of MMSE are much better.

The complexity of a linear receiver is composed of  the complexity of finding the appropriate matrix $\bB$ and the multiplying operation $\bB \by$. For the general case, the more complex part is finding $\bB$. In both ZF and MMSE finding $\bB$ depended on inverting a matrix. Hence, both have the same asymptotic complexity. In order to find $\bB$, the linear receiver must know the channel $\bH$, since $\bB$ is a function of the channel realization.
 
Knowing CSI in both transmitter and receiver may help, only if different power allocations may be used. If this is the case, then, by using SVD, the transmissions can be ''directed'' to orthogonal directions, such that the capacity of the channel can be achieved by SISO receivers, since the channel becomes a set of parallel, independent scalar Gaussian sub-channels \cite[7.1.1]{tse2005fundamentals}.






%When trying to maximize the SINR, it only makes sense to look at both noise and interference together as Gaussian noise. However, unlike white noise, this noise may be correlated. We model it by:
%\begin{align*}
%\by= \bh x+\bx
%\end{align*}
%Where $\bz$ is complex noise with covariance matrix $\bK_z$. The other parameters remain unchanged. $\bx$ and $\bz$ assume to be uncorrelated. What is the filter that would maximize the SNR? If $\bz$ is white noise, i.e., $\bK_z=\bI$, we know that optimal thing to do it project it over $\bh$. Otherwise, it is needed to be whiten, which is done by applying $\bK_z^{-\frac{1}{2}}$ over $\by$. 
%\begin{align*}
%\tilde{\by} = \bK_z^{-\frac{1}{2}}\by = \bK_z^{-\frac{1}{2}}\bh x + \tilde{\bz} = \tilde{\bh}x + \tilde{\bz}
%\end{align*}
%Where $\tilde{\bz}$ is white noise. Now, the optimal thing to do in to project $\tilde{\by}$ to the direction of $\tilde{\bh}$, resulting in a scalar channel. 
%Let \begin{align*}
%&\bb_{mmse} = \bK_z^{-1}\bh\\
%&\bB_{mmse} = \bK_z^{-1}\bH\\
%\end{align*} 
%
%
%Note that for the channel above: 
%\begin{align*}
%\bK_{z_k} = N_0\bI_{n_r} + \sum_{i\neq k}^{n_t} P_i\bh_i\bh_i^* 
%\end{align*}
%When all the transmission powers equal $P$  we have:
%\begin{align*}
%\bK_{z_k} = N_0\bI_{n_r} + P\bH\bH^*
%\end{align*}
%The SINR of the $k^{th}$ stream is 
%\begin{align*}
%SINR_{MMSE} =P_k\bh_k^*\left(N_0\bI_{n_r} + P\bH\bH^*\right)^{-1}\bh_k
%\end{align*}
%For equal transmigration powers and when $N_0=1$the SINR of MMSE becomes:
%\begin{align*}
%SINR_{MMSE} 
%& = P\bh_k^*\left(\bI_{n_r} + \sum_{i\neq k}^{n_t} P\bh_i\bh_i^*\right)^{-1}\bh_k\\
%& = \bh_k^*\left(\frac{1}{P}\bI_{n_r} + \sum_{i\neq k}^{n_t} \bh_i\bh_i^*\right)^{-1}\bh_k\\
%\end{align*}
%Note that for small $P$ values, $\bK_{z_K} \approx N_0\bI$, which is the match filter. For high values, on the other hand, it becomes decorrelator.
%
%\subsubsection{MMSE SIC}
%Using the SIC idea. The MMSE-SIC achieves the MIMO capacity; Assume that both $\bx$ and $\bz$ are Gaussian. 
%\begin{align*}
%I(\bx;\by) &=  
%I(x_1,\ldots,x_{n_t};\by) = I(x_1;\by) + \sum_{i=2}^{n_t} I(x_i;\by \lvert  x_1,\ldots,x_{i-1}  )
%\end{align*}
%Let 
%\begin{align*}
%\acute{\by_1} &= \by \\
%\acute{\by_k} &= \by - \sum_{i=1}^{k-1}\bh x_i = \bh_k x_k + \sum_{i>k}\bh_i x_i +\bw
%\end{align*}
 %The $k^{th}$ term in the chain rule is:
%\begin{align*}
%I(x_k;\by \lvert  x_1,\ldots,x_{k-1} ) 
%& = I(x_k;\bw + \sum_{i=1}^{n_t} \bh_i x_i\lvert  x_1,\ldots,x_{k-1} )  \\ 
%& = I(x_k;\bw + \bh_k x_k + \sum_{i=k+1}^{n_t} \bh_i x_i ) = I(x_k;\acute{\by_k} )\\
%& = I(x_k;\bv_{mmse,k}^* \acute{\by_k} )
%\end{align*}
%Which means that given $\bv_{mmse,k}^* \acute{\by_k}$, $\by$ and $\{x\}_{i=1}^k$ are independent. Noting that $ I(x_k;\bv_{mmse,k}^* \acute{\by_k} )$ is exactly the rate achieved by the $k^{th}$ stream when use MMSE-SIC, so all stream together achieve a sum rate of 
%\begin{align*}
%\sum_{i=1}^{n_t} I(x_i ; \bv_{mmse,i}^* \acute{\by_i}) = I(\bx,\by)
%\end{align*}
%Hence, MMSE-SIC achieves the sum rate capacity.

==> tex_files/1_preliminaries/model.tex <==
\section{Channel Model}
We consider a MIMO Channel with $n_t$ transmitting antennas and a base station (BS) equipped with $n_r$ receiving antennas. In particular, we consider the uplink model, where each transmit antenna belongs to a single user who was chosen arbitrary. Users do not cooperate with the others. This model is also known as Multiple-User Single-Input-Multiple-Output (MU-SIMO). \Cref{fig:MU_SIMO} depicts the setting. We assume that $1\leq n_t \leq n_r$.  When the $n_t$ users are transmitting simultaneously, each sub channel from a transmitting antenna $t_i$ to a receiving antenna $r_j$ is represented by $h_{ij} \in \C$.
\begin{figure}[ht]
	\centering
		\includegraphics[width=0.4\textwidth]{dependencies/fig/MIMO_scheme_sketch/MU_SIMO.pdf}
	\caption{Five users, each  equipped with a single antenna, are transmitting to a single BS.}
	\label{fig:MU_SIMO}
\end{figure} 

Throughout this work, we will use boldface lowercase to refer vectors, e.g., $\bh_i = [h_{i1},h_{i2},\ldots,h_{i n_r}]^T \in \C^{n_r}$  represents the channel vector of the $i^{th}$ user to the BS. Boldface uppercase are used to refer to matrices, e.g., the channel matrix between the users to the BS is denoted by $\bH = [\bh_1,\bh_2,\ldots,\bh_{n_t}] \in \C^{n_r \times n_t}\in \C^{n_r \times n_t}$. It is common to assume that the entries of $\bH$ are i.i.d complex Normal RVs, e.g., \cite[Chapter 2]{tse2005fundamentals}. In this work  we assume unit variance. We further assume that the receiver has a channel state information (SCIR), i.e., the channel $\bH$ is known to the receiver. 

The signal transmitted by the i'th user is  $x_i \in \C$. At the receiving antennas, we assume i.i.d complex Normal noise with variance $N_0$, which is denoted by $\bz \in \C^{n_r}$. Accordingly, $\by \in \C^{n_r}$, the received vector at the BS is
\begin{equation}
\by=\bH \bx+\bz,
\end{equation}
where $\bx = [x_1, \ldots, x_{n_t}]^T \in \C^k$ is the transmitted vector. The average transmission power of each user is bounded by $P$. \Cref{fig:channel_diagram} depicts the channel model.
\begin{figure}[ht]
	\centering
		\includegraphics[width=0.4\textwidth]{dependencies/fig/MIMO_scheme_sketch/MIMO_scheme.pdf}
	\caption{Channel diagram. $\{m_i\}$ represent the information bits while $\{x_i\}$ stand for the code words (symbols). Enc is the encoder which performs the transformation from  $\{m_i\}$  to $\{x_i\}$.} 
	\label{fig:channel_diagram}
\end{figure}






==> tex_files/1_preliminaries/preliminaries_file.tex <==
\section{Integer Forcing}
The key idea of \emph{Integer-forcing} is to look at the linear combination of the original messages forced by the channel as a new message, and decode it. E.g., if the receiver $y_j$, i.e, the B.S $j$'s receiving antenna, wants to decode only the first message $x_1$, instead of considering all the other message $\{x_i\}_{i=2}^{k}$ as interference i.e., unwanted noise, $y_j$ will try to decode 	 $\sum \limits_{1 \leq i \leq k} {f({h_{ji})}x_i}$, where $f(\cdot)  \in \N$ is some known deterministic function that can be chosen. For example, if $\forall i,j: h_{ji} \in \N$ and all the lines of \textbf{H} are linearly independent, then choosing $f(h_{ji})=h_{ji}$ is possible. This point of view allows $y_j$ to use all the messages to increase the signal power, ignore the interferences (other messages are now part of the wanted new message), while keeping the noise unchanged, which may increase the SNR at the receiver . At this part, each new message is represented as linear combination of integers (original messages) with integer coefficients ($f(h_{ji})$) \footnote{Therefore, is also an integer}. Only after the noise is removed, $y_j$, using the other messages which where decoded by the other receivers, can remove the other irrelevant messages and keep $x_1$. At this part of the decoding process, there is no noise, which means all the possible new messages (words) to be decoded are over a finite alphabet. Since all those words are linear combinations, each word can be represented as a vector of coefficients, and all the words together can be represented as a matrix. The information gathering from other receivers and the decoding of the wanted (original) message  is a digital process which involves finding the inverse of the words-matrix. 

In \cite{nazer2011compute} a single letter expression for the ''Computation Rate'' can be found. The ''Computation Rate'' is the maximal possible rate, for a decode-able transmission, using a specific linear (integer) combination. The expression for the "Computation Rate" for the m'th user is given by:
\begin{equation}
\label{eq:COMP_rate_user_beta_one}
			R_{comp}(\bh_m,\ba_m) =\frac{1}{2}\posLog[   \frac{P}{ 1+P \normSqr[\bh_m-\ba_m] }   ]
	\end{equation}
	
	Where $\ba_m$ is the coefficients vector of the m'th equation to be decoded and $\bh_m$ is the channel gains of the m'th user. 
	
	One way to look at the $1+P\normSqr[\bh_m-\ba_m]$ expression is as an effective noise; The ''1'' stands for the channel noise which $\sim  \mathcal{N} (0,1) $, while the $P\normSqr[\bh_m-\ba_m]$ part can be explained as a quantization noise. The bigger the distance between the equation and channel gains is, the less efficient this equation decoding is. The channel gains are continuous, but the equation coefficients are discrete, which means that in addition to the channel noise, there is also a quantization noise effect caused by the quantization of the channel. The the previous happens because more power is invested in a interfering direction. 

In order to reduce the quantization noise effect, the channel output can be multiply by vector. I.e, the i'th antenna can multiply $y_i$ by a vector $\bb_i$ and the output vector $\by$ can be multiply by a matrix $\bB$. This multiplication may help ''moving'' the channel actual values closer in norm to the desired integer values, however, it also causes the noise variance multiplication by $\beta^2$. For $\beta \gg 1$ it might be a problem.


For a given $\bb_m\in\R^r$, the Computation Rate of the m'th user is now given by:
\begin{equation}
\label{eq:COMP_rate_user_beta}
			R_{comp}(\bH,\ba_m,\bb_m) =\frac{1}{2}	\posLog[   \frac{P}{ \normSqr[\bb_m]+P \normSqr[\bH^T\bb_m-\ba_m] }   ]
	\end{equation}
	
This equation shows that there is a balance between minimizing the noise power to minimizing the quantization noise. For example, if a very big $\beta_{zero}$ value gives a zero quantization noise corresponding to some $\ba$, it might be a better idea to choose  $\beta_{n-zero} < \beta_{zero}$ for $\tilde{\ba}$. Even though $\beta_{n-zero}$ causes a non-zero quantization noise, the noise power amplification, which equals to $\beta_{n-zero}^2$, is now smaller. For $\beta_{n-zero} \ll \beta_{zero}$, the current effective noise, relatively to the one caused by $\beta_{zero}$, is much smaller. Another conclusion from this equation is that for different transition powers there might be different tuples $(\beta_1,\ba_1 )$ and $(\beta_2, \ba_2)$ causing the effective noise to be minimal and the $	R_{comp}$ to be maximal. The above is correct because the higher the transmission power is, the bigger the percentage of quantization noise out of the entire effective noise.

In order to complete the computation, each equation is shared by all the users after the decoding process, only then, all the equations can be solved, The last action is resulted by knowing all the original messages. This process works if all the users share the some code book. Since the logarithm of amount of code words in a code book is equivalent to the code rate, all users need to transmit at the same rate, allowing the same code book to be shared by all. An achievable rate is a rate such that:
$\forall \bh_m \in \bH$, 
$\forall \ba_m \in \bA$, 
$\forall \bb_m \in \R^r$
 where 
, $\bB$= $[\bb_1, \ldots,\bb_k]^T \in \R^{k \times r}$, $\bA \in \Z^{k \times k} = [\ba_1,\ba_2, \ldots,\ba_k]^T$ 

%the rate $	R_{comp}(\bH,\bA,\bB)$ is achievable for all the decoders, i.e, $\forall i \in \makeSet[1, \ldots k], y_i$ can be decoded.


	\begin{equation}
\label{eq:COMP_rate}
			R_{comp}(\bH,\bA,\bB) =
	\end{equation} 
	
		\begin{equation*}
\frac{1}{2} \min\limits_{m \in \makeSet[1,\ldots, k]}\posLog[\frac{P}{\normSqr[\bb_m]+P\normSqr[\bH^{T}\bb_m-\ba_m]}]
	\end{equation*}
	
	Note that $\ba_m$ is a vector where each of it's elements $\ba_{m[i]}$ is the coefficient of its responding variable $x_i$ (the i'th message) to be decoded. E.g., if $\ba_1 = [3, 2]^T$, $y_1$ will try to decode the following equation: $3x_1 + 2x_2$
	
	The IF rate is achievable by optimization over all the possible full rank $\bA$ and all the matrices $\bB$:
\begin{equation}
\label{eq:IF_rate}
R_{IF}(\bH) =
 k\cdot \max\limits_{\bA \in \Z^{k \times k} }  \max\limits_{\bB \in \R^{k \times r}}{R_{comp}(\bH,\bA,\bB)}
	\end{equation} 
	
	
	Given $\bH$ and $\bA$, finding $\bB_{opt}$, as explained in  \cite{zhan2014integer}, can be done by:
\begin{equation}
\label{eq:find_B_opt}
			\bB_{opt} = P {\ } \bA\bH^T(\bI+P {\ } \bH\bH^T)^{-1}
	\end{equation} 


Another way to look at $R_{comp}$ is by looking at the effective SNR.
I.e, the ratio between the transmitted power and the optimal effective noise which, for the m'th antenna.	Therefore, IF can be represented by:
		\begin{equation}
\label{eq:RIFNoiseRepresentation}
	R_{IF}(\bH)= k\cdot \max\limits_{\bA \in \Z^{k \times k} }R_{comp}(\bH,\bA,\bB_{opt})
	\end{equation} 
	


	\begin{equation}
\label{eq:RcompNoiseRepresentation}
R_{comp}(\bH,\bA,\bB_{opt}) = \min\limits_{k=1 \ldots K}\frac{1}{2}\posLog[\frac{P}{\sigma_{opt,m}^2}]
	\end{equation} 



	\begin{equation}
\label{eq:effNoise}
			\sigma_{opt,m}^2= P\cdot \ba_m^T(\bI-P \cdot\bH^T(\bI+P\cdot\bH\bH^T)^{-1}\bH)\ba_m
	\end{equation} 
	
	
	In order to make the search of $\bA$ more efficient, the following constraint on $\bA$ vectors is given in \cite{zhan2014integer}: 
	\begin{equation}
\label{eq:normConstrintLowP}
		\forall \ba_m\in\bA: \|a_m\|<1+\sqrt{P}\cdot\lambda_{max}(\bH) \footnote{$\lambda_{max}(\bH)$ is the biggest eigenvalue of $\bH\bH^T$  }
	\end{equation} 	

==> tex_files/bounds_on_eff_snr/bounds_on_eff_snr_IF.tex <==
\subsection{Bounds On The Effective SNR of the IF Scheme }\label{subsec:bound_eff_snr_if}

\reminder{This subsection can be removed since both upper and lower bound here are less tight then Or's in \cite{ordentlich2015precoded}. The only interesting part is when we extend Or's upper bound from IF to B-IF, which happens in the next subsection any way.}

Here we present upper and lower bounds on the effective SNR of IF. Recalling that the effective SNR of IF is defined as the effective SNR of the worst vector. Both bounds are less tight then those in \cite{ordentlich2015precoded}, however, achieve the same asymptotic value. The main advantage of the bounds in this work over the bounds in \cite{ordentlich2015precoded}, lies in the fact that the lower bound for the same channel for different values of P, $P_1$ and $P_2$, is a factor of $\frac{P_1}{P_2}$. Thus, for a simulation with different values of P, the bound can be calculated only once, instead for each value of $P$.

Let $\bA_{LB}^{opt} \in \Z^{M_T \times M_T}$ be the optimal matrix for the lower bound; it is a full ranked integer matrix such that its worst vector achieves the highest rate out of all the possible $\bA$ matrices. Hence,
\begin{align}
\begin{split}
\bA_{LB}^{opt}  &= \argmax_{\bA \in \Z^{M_T \times M_T}} \min_{k \in \{1,\ldots,M_T \}} 
\frac{P}{\ba^T(\bH^T\bH)^{-1}\ba}\\ 
& = P \cdot \argmin_{\bA \in \Z^{M_T \times M_T}} \max_{k \in \{1,\ldots,M_T \}}
\ba^T\bS^{-1}\ba.
\end{split}
\end{align}
The matrix $\bS^{-1} = \left(\bH\bH^T\right)^{-1}$ is symmetric and positive definite almost surly, hence can be expressed as
\begin{equation}
\bS^{-1} = \bL\bL^T,
\end{equation}
by the Cholesky decomposition, where $\bL$ is a lower triangular matrix with strictly positive diagonal entries. Thus, 
\begin{equation}
\bA_{LB}^{opt} = P \argmin_{\bA \in \Z^{M_T \times M_T}} \max_{k \in \{1,\ldots,M_T \}}  \normSqr[\bL^T\ba].
\end{equation}

\begin{definition}[Successive minima]\label{def:successive_minima}
According to \cite[Definition 1]{ordentlich2015precoded}, let $\Lambda(\bG)$ be a lattice spanned by the full-rank matrix $\bG \in \R^{K \times K}$. For $k = 1,\ldots,K$,  the $k^{th}$ successive minima is defined as 
\begin{equation*}
\lambda_k(\bG) \defined \inf \left\{r : \dim \left( span \left(\Lambda(\bG) \bigcap \mathcal{B}(0,r)  \right) \right) \geq k  \right\},
\end{equation*}
where $\mathcal{B}(0,r) = \{ \bx\in \bR^K : \|\bx\| \leq r \}$ is the closed ball of radios $r$ around 0.   
\end{definition}

\begin{definition}[Dual lattic] For a lattice $\Lambda(\bG)$ with a generating full-rank matrix $\bG \in \R^{K \times K}$, the dual lattice is defined by
\begin{equation*}
\Lambda^*(\bG) \defined \Lambda((\bG^{T})^{-1})
.
\end{equation*}
\end{definition}

\subsubsection{Lower Bound On The Effective SNR of IF}\label{ssc:LB_eff_snr_if}

According to the \Cref{def:successive_minima}, the lower bound for the effective SNR can be expressed as
\begin{equation}
LB(\bH) = \frac{1}{\lambda_{M_T}^2(\bL^T)}.
\end{equation}
In order to bound the $M_T$ th successive minima, exactly as in \cite{ordentlich2015precoded}, the transference theorem by Banaszczyk \cite{banaszczyk1993new} is used.

\begin{theorem}[Theorem 2.1, \cite{banaszczyk1993new}]\label{trm:dual_lattice}
Let $\Lambda(\bG)$ be a lattice with a full-rank generating matrix $\bG \in \R^{K \times K}$ and let $\Lambda^*(\bG) =\Lambda((\bG^{T})^{-1})$ be its dual lattice. The successive minima of $\Lambda(\bG)$ and  $\Lambda^*(\bG)$ satisfy the following inequality 
\begin{equation*}
\lambda_k(\bG)\lambda_{K-k+1}((\bG^T)^{-1})<K,  \quad  \forall k \in 1,\ldots,K. 
\end{equation*}
\end{theorem}
\begin{proof}See \cite{banaszczyk1993new}. \end{proof}


According to \cite[Remark 4]{ordentlich2015precoded},
\begin{equation*}
SNR_{eff}(\bH) > \frac{1}{M_T^2} \min_{\ba \in \Z^{M_T} \setminus \mathbf{0}} \left\{\normSqr[\ba] + P\ba^T\bH^T\bH\ba  \right\}.
\end{equation*}
\begin{remark}
Let us denote $\ba_{min}$ by
\begin{equation*}
\ba_{min} =\argmin_{\ba \in \Z^{M_T} \setminus \mathbf{0}} \left\{\normSqr[\ba] + P\ba^T\bH^T\bH\ba  \right\}.
\end{equation*}
Then, it is not hard to see why
\begin{align*}
 &\frac{1}{M_T^2} \min_{\ba \in \Z^{M_T} \setminus \mathbf{0}} \left\{\normSqr[\ba] + P\ba^T\bH^T\bH\ba  \right\}\\ 
&- \quad \frac{P}{M_T^2} \min_{\ba \in \Z^{M_T} \setminus \mathbf{0}} \left\{\ba^T\bH^T\bH\ba  \right\}\\
& \leq \frac{\normSqr[\ba_{min}]}{M_T^2}.
\end{align*}
By \cref{eq:bound_the_norm_of_a}
	\begin{equation*}
		\forall \ba_k\in\bA: \|\ba_k\|<1+\sqrt{P}\cdot\lambda_{max}(\bH).
	\end{equation*} 	
Therefore, when $P \rightarrow 0 \Longrightarrow \forall k:\normSqr[\ba_{k}]=1$ and the difference between the bounds is bounded by $\frac{1}{M_T^2}$. 
 \end{remark}

\begin{remark}
 By denoting  \begin{align*}\ba_{min}=\argmin_{\ba \in \Z^{M_T} \setminus \mathbf{0}} \left\{\normSqr[\ba] + P\ba^T\bH^T\bH\ba  \right\}\end{align*} we have,
\begin{align*}
&\frac{\normSqr[\ba_{min}] + P\ba_{min}^T\bH^T\bH\ba_{min}}{{\frac{P}{M_T^2} \min_{\ba \in \Z^{M_T} \setminus \mathbf{0}} \left\{\ba^T\bH^T\bH\ba  \right\}} } \leq\\
 &\leq \frac{\normSqr[\ba_{min}] + P\ba_{min}^T\bH^T\bH\ba_{min}}{P\ba_{min}^T\bH^T\bH\ba_{min}}\\
&= \frac{\frac{\normSqr[\ba_{min}]}{P} + \ba_{min}^T\bH^T\bH\ba_{min}}{\ba_{min}^T\bH^T\bH\ba_{min}}\\
&= 1+ \frac{\normSqr[\ba_{min}]}{P\ba_{min}^T\bH^T\bH\ba_{min}}\\
&= 1+ \frac{1}{P\frac{\ba_{min}^T}{\|\ba_{min}\|}\bH^T\bH\frac{\ba_{min}}{\|\ba_{min}\|}}\\
&\leq 1+ \frac{1}{P\lambda_{min}(\bH)} \stackrel{P\rightarrow \infty}{\longrightarrow} 1,
\end{align*}
concluding that both bounds achieve the same asymptotic rate.
 \end{remark}


\subsubsection{Upper Bound On The Effective SNR of IF}\label{SSC:UB_eff_SNR_IF}
\begin{claim}\label{claim:LB_sec_minima}
Let $\Lambda(\bG)$ be a lattice with a full-rank generating matrix $\bG \in \R^{K \times K}$ and let $\Lambda^*(\bG) =\Lambda((\bG^{T})^{-1})$ be its dual lattice. The successive minima of $\Lambda(\bG)$ and  $\Lambda^*(\bG)$ satisfy the following inequality 
\begin{equation*}
\lambda_k(\bG)\lambda_{K-k+1}((\bG^T)^{-1})>1,  \quad  \forall k \in 1,\ldots,K 
\end{equation*}\end{claim}
\begin{proof} See [\cite{cassels2012introduction}, VIII.5, Theorem VI].\end{proof}



==> tex_files/bounds_on_eff_snr/bounds_on_eff_snr_IF_block_schemes.tex <==
\subsection{Upper Bound On The Effective SNR of B-IF }\label{subsec:bound_eff_snr_if_b}
Let us assume that there is no interference between different blocks, i.e., each block is an independent IF scheme of two transmitters. In that case, $\bS$ is also a block matrix. For example, when $M_T=4$, $\bS$ becomes:
$\begin{bmatrix} \bS_1& \mathbf{0}  \\ \mathbf{0} & \bS_2 \end{bmatrix}$ where $\bS_i \in \R^{2 \times 2}$. Using the same method as in \cite{ordentlich2015precoded}, the effective SNR of the $i^{th}$ block can be bounded by 
\begin{equation*}
\min_{\ba \in \Z^2 \setminus \mathbf{0}} \ba^T (\bI + P \bS_i)\ba,
\end{equation*}
where $i \in \{1,2\}$.

\begin{equation}
\min_{\ba_i} \ba_i^T (\bI + P \bS_i)\ba_i= \min_{\tilde{\ba} } \ba^T (\bI + P \bS)\ba,
\end{equation}
where $\ba_i  \in \Z^2 \setminus \mathbf{0}$ and $\tilde{\ba} = [\hat{\ba}, 0 ,0]^T$ such that  $\hat{\ba}  \in \Z^2 \setminus \mathbf{0}$. Note that $\tilde{\ba} \subset \Z^{4}\setminus \mathbf{0}$. Thus, 
\begin{equation}
\min_{\ba \in \Z^2 \setminus \mathbf{0}} \ba^T (\bI + P \bS_i)\ba \geq \min_{\ba \in \Z^4 \setminus \mathbf{0}} \ba^T (\bI + P \bS)\ba
\end{equation}
which is the upper bound on IF.

==> tex_files/bounds_on_eff_snr/bounds_on_eff_snr_single_equation_bck.tex <==
Our first result is a lower bound.
\begin{theorem}\label{lem:LB_lower_bounds_SNR_eff}
Let $\ba \in \Z^{M_T}$ s.t.\ $\normSqr[\ba]>0$. Then,
\begin{equation}
SNR_{eff}(\bH,\ba) \geq {\left({  \ba^T\left({P\bH^T\bH}\right)^{-1}\ba }\right)^{-1}}.
\end{equation}
\end{theorem}
The intuition behind \Cref{lem:LB_lower_bounds_SNR_eff} comes from the fact that  $\bH^T\bH$ is almost surely a positive definite matrix. Hence, $\frac{\left({\ba^T \left(\bI+P\bH^T\bH\right)^{-1}\ba}\right)^{-1}}{\left({  \ba^T\left({P\bH^T\bH}\right)^{-1}\ba }\right)^{-1}}$
 is a ratio between quadratic forms of the inverses of positive definite matrices. Intuitively, $\bI$, which appears in the effective SNR, enlarges the singular values of the corresponding quadratic form. The complete proof, as well as other proofs in this paper and detailed technical discussions can be found in the Appendix, \Cref{sec:appendix}.

\begin{definition}\label{def:LB_def}
$LB(\bH,\ba) \defined \left({  \ba^T(P\bH^T\bH)^{-1}\ba }\right)^{-1} = \frac{P}{\ba^T\bS^{-1}\ba}$, where $\bS = \bH^T\bH$.
\end{definition}
When $\ba$ is fixed, the distribution of this lower bound can be computed. 
\begin{corollary}\label{corl:LB_distribution}
For a fixed $\ba$, the lower bound on the effective SNR has the following gamma distribution
\begin{align}
LB(\bH,\ba) \sim \Gamma\left(\frac{M_R-M_T+1}{2},\frac{2P}{\normSqr[\ba]}\right). \label{eq:LB_distribution}
\end{align}
\end{corollary}
The proof is a consequence of \cite[proposition 8.9]{eaton}, combined with the connection between the $\chi^2$ and the $\Gamma$ distributions.

Note that due to the $\frac{1}{\normSqr[\ba]}$ factor, without CSI the best vector of coefficients for the lower bound is a unit vector $\be_i$. Hence, the best choice without CSI is $\bA = \bI$. In that case, the lower bound is distributed exactly like ZF \cite[Lemma 1]{li2006distribution}, and IF becomes MMSE. Note also that the dimensions of $\bH$ do not effect the distribution, only the difference between the number of rows and the number of columns.
%

We now turn to a corresponding upper bound.
\begin{theorem}\label{lem:UB_eff_snr}
Let $\ba\in\Z^{M_T}$ s.t $\normSqr[\ba]>0$. Then, 
\begin{equation}
SNR_{eff}(\bH,\ba) \leq P\left({\ba^T{\bS}^{-1}\ba }\right)^{-1} \sum_{k=0}^\infty \left(\frac{tr(\bS^{-1})}{P}\right)^k . 
\end{equation}
\end{theorem}
\begin{proof}[Proof of \Cref{lem:UB_eff_snr}]
The proof of \Cref{lem:UB_eff_snr} is directly from \Cref{clm:LB_ratio_IF_vs_my_known_dist} by setting $M=\bH^T\bH$ and $\epsilon = \frac{1}{P}$. 
\end{proof}

Note that the lower bound times an infinite series is exactly the upper bound. Thus, setting 
\begin{equation}
C(\bH,P) \defined \sum_{k=0}^\infty \left(\frac{tr(\bS^{-1})}{P}\right)^k, 
\label{eq:def_of_C}
\end{equation}
we have 

\begin{align*}
P\left({\ba^T{\bS}^{-1}\ba }\right)^{-1} \sum_{k=0}^\infty \left(\frac{tr(\bS^{-1})}{P}\right)^k=LB(\bH,\ba) \cdot C(\bH,P)
\end{align*}
and hence,

\begin{align}\label{eq:LB_and_UB_to_SNR_eff}
LB(\bH,\ba) \leq SNR_{eff}(\bH,\ba)
& \leq C(\bH,P)\cdot LB(\bH,\ba).
\end{align}
\normalsize

On one hand, there always exists a non-zero probability for the series above not to converge. In that case, the upper bound is meaningless. On the other hand, it is not hard to see that when $tr(\bS^{-1})<P$, $C(\bH,P) =\frac{1}{1-\frac{tr(\bS^{-1})}{P}}$.
Hence, $1\leq \frac{SNR_{eff}(\bH,\ba)}{LB(\bH,\ba)} \leq \frac{1}{1-\frac{tr(\bS^{-1})}{P}}$.
Note that when $P\rightarrow \infty$, $\frac{tr(\bS^{-1})}{P} \longrightarrow 0$. Thus, when $P\rightarrow\infty$, the lower and upper bounds are tight.
\begin{figure}
    \centering
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width=\textwidth]{dependencies/fig/bounds/LB_and_UB/LB_SNR_eff_10dB.pdf}
        \caption{Lower bound on effective SNR.}
        \label{fig:LB_SNR_eff_Mt_2_Mr_2}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \includegraphics[width=\textwidth]{dependencies/fig/bounds/LB_and_UB/UB_SNR_eff_10dB.pdf}
        \caption{Lower and upper bounds for a finite upper bound.}
        \label{fig:UB_SNR_eff_Mt_2_Mr_2}
    \end{subfigure}
   	\caption{CDF of the $SNR_{eff}(\bH,\be_1)$ together with its lower and upper bounds for $M_R=M_T=2$ and when $P=10dB$.  }
	\label{fig:LBAndUB_SNR_eff_Mt_2_Mr_2}
\end{figure}

\Cref{fig:LBAndUB_SNR_eff_Mt_2_Mr_2} depicts the CDF of the effective SNR for $M_R$=$M_T$=2 and for $P$=$10$dB along side with its upper and lower bounds. Note that even though the same parameters where used in both sub-figures, their behavior is different, since in \cref{fig:UB_SNR_eff_Mt_2_Mr_2} we plot only the channels for which $C(\bH,P)< \infty$, i.e., $tr(\bS^{-1}) = \sum\frac{1}{d_i}< P$. Higher singular values are associated with higher capacity,  thus demanding that the sum of their \emph{inverses} is smaller than $P$ is basically enforcing usage of better channels.

